Pix2NeRF: Unsupervised Conditional $\pi$-GAN for Single Image to Neural Radiance Fields Translation

We propose a pipeline to generate Neural Radiance Fields~(NeRF) of an object or a scene of a specific class, conditioned on a single input image. This is a challenging task, as training NeRF requires multiple views of the same scene, coupled with corresponding poses, which are hard to obtain. Our method is based on $\pi$-GAN, a generative model for unconditional 3D-aware image synthesis, which maps random latent codes to radiance fields of a class of objects. We jointly optimize (1) the $\pi$-GAN objective to utilize its high-fidelity 3D-aware generation and (2) a carefully designed reconstruction objective. The latter includes an encoder coupled with $\pi$-GAN generator to form an auto-encoder. Unlike previous few-shot NeRF approaches, our pipeline is unsupervised, capable of being trained with independent images without 3D, multi-view, or pose supervision. Applications of our pipeline include 3d avatar generation, object-centric novel view synthesis with a single input image, and 3d-aware super-resolution, to name a few.

==> tab/srnchairs_ablations.tex <==
\begin{table}[h!]
\centering
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{@{}lccc@{}}
\toprule
& \multicolumn{3}{c}{64 $\times$ 64}\\
Method & FID $\downarrow$ & KID $\downarrow$ & IS $\uparrow$ \\
\midrule
\textbf{A} & 34.01 & 1.73 & 3.65 \\
\textbf{B} & 43.06 & 2.49 & 2.92 \\
\textbf{C} & 41.47 & 2.80 & 2.96 \\
\textbf{D} & 35.72 & 1.74 & 3.75 \\
\textbf{E} & 21.67 & 0.89 & 4.35 \\
\textbf{F} & 27.70 & 1.22 & 4.09 \\
\textbf{G} & 27.10 & 1.31 & 4.26 \\
\textbf{H} & 41.11 & 2.27 & 3.34 \\
\textbf{I} & 184.10 & 17.19 & 2.55 \\
\textbf{J} & 266.64 & 30.29 & 1.98 \\
\midrule
Pix2NeRF conditional & \textbf{17.55} & \textbf{0.59} & \textbf{4.36} \\
\bottomrule
\end{tabular}
}

\resizebox{0.7\linewidth}{!}{
\begin{tabular}{@{}lcc@{}}
\toprule
& \multicolumn{2}{c}{64 $\times$ 64}\\
Method & PSNR $\uparrow$ & SSIM $\uparrow$\\
\midrule
\textbf{A} & 15.91 & 0.71\\
\textbf{B} & 16.27 & 0.71\\
\textbf{C} & 15.14 & 0.68\\
\textbf{D} & 16.81 & 0.77\\
\textbf{E} & 18.03 & 0.79\\
\textbf{F} & 16.98 & 0.77\\
\textbf{G} & 17.77 & 0.79\\
\textbf{H} & 14.98 & 0.74\\
\textbf{I} & 10.95 & 0.59\\
\textbf{J} & 10.28 & 0.47\\
\midrule
Pix2NeRF conditional & \textbf{18.75} & \textbf{0.82}\\
\bottomrule
\end{tabular}
}
%
\caption{
% 
Ablation studies quantitative results on ShapeNet-SRN~\cite{angel2015shapenet, sitzmann2019srns}.
% 
}
\label{tab:srnchairs_ablations}
\end{table}%
